Entropic Optimal Transport between Unbalanced Gaussian Measures has a Closed Form

Although optimal transport (OT) problems admit closed form solutions in a very few notable cases, e.g. in 1D or between Gaussians, these closed forms have proved extremely fecund for practitioners to define tools inspired from the OT geometry. On the other hand, the numerical resolution of OT problems using entropic regularization has given rise to many applications, but because there are no known closed-form solutions for entropic regularized OT problems, these approaches are mostly algorithmic, not informed by elegant closed forms. In this paper, we propose to fill the void at the intersection between these two schools of thought in OT by proving that the entropy-regularized optimal transport problem between two Gaussian measures admits a closed form. Contrary to the unregularized case, for which the explicit form is given by the Wasserstein-Bures distance, the closed form we obtain is differentiable everywhere, even for Gaussians with degenerate covariance matrices. We obtain this closed form solution by solving the fixed-point equation behind Sinkhorn's algorithm, the default method for computing entropic regularized OT. Remarkably, this approach extends to the generalized unbalanced case -- where Gaussian measures are scaled by positive constants. This extension leads to a closed form expression for unbalanced Gaussians as well, and highlights the mass transportation / destruction trade-off seen in unbalanced optimal transport. Moreover, in both settings, we show that the optimal transportation plans are (scaled) Gaussians and provide analytical formulas of their parameters. These formulas constitute the first non-trivial closed forms for entropy-regularized optimal transport, thus providing a ground truth for the analysis of entropic OT and Sinkhorn's algorithm.

==> sections/brouillon.tex <==
\section{Brouillon}

\subsection{Entropy Regularization}\BM{which regularization should we use?}

\begin{align}
V &\leftarrow B\oplus(-U - \sigma^2 \Id)\\
v &\leftarrow V(B^{-1}b - (U + \sigma^2 \Id)^{-1}u)
\end{align}

followed by

\begin{align}
U &\leftarrow A\oplus(-V - \sigma^2 \Id)\\
u &\leftarrow U(A^{-1}a - (V + \sigma^2 \Id)^{-1}v)
\end{align}

\begin{align}
    H_2^{-1} = 
    \begin{pmatrix} 
        U^{-1} +  \frac{1}{\sigma^2} \Id & - \frac{1}{\sigma^2} \Id \\
         -  \frac{1}{\sigma^2} \Id  & V^{-1} + \frac{1}{\sigma^2} \Id\\
    \end{pmatrix}
\end{align}

Hence 

\begin{align}
    H_2 = 
    \begin{pmatrix} 
        U\oplus(V +  \sigma^2 \Id) & \frac{1}{\sigma^2}(U \oplus (V +  \sigma^2 \Id) \left(V\oplus (U +  \sigma^2 \Id)\right)^{-1} \\
         \frac{1}{\sigma^2}\left(V\oplus (U +  \sigma^2 \Id)\right)^{-1}(U\oplus(V + \sigma^2 \Id)) & V\oplus (U +  \sigma^2 \Id)\\
    \end{pmatrix}
\end{align}








\begin{algorithm}[H]
\caption{Sinkhorn Iterations (Relative Entropy)}\label{alg:sinkhorn}
\begin{algorithmic} 
\REQUIRE $\bA, \bB \in \PD$, $\bU \in \PD$ $\bu \in \RR^d$,  $\sigma^2 > 0$
\WHILE{not converged}
\STATE $\bV \leftarrow - \bU\oplus \bA - \sigma^2\Id$
\STATE $\bv \leftarrow -(\bV + \sigma^2\Id)(\bA^{-1}\ba + \bU^{-1}\bu)$
\STATE $\bU \leftarrow - \bV\oplus \bB - \sigma^2\Id$
\STATE $\bu \leftarrow -(\bU + \sigma^2\Id)(\bB^{-1}\bb + \bV^{-1}\bv)$
\ENDWHILE
\ENSURE $\bU, \bu, \bV, \bv$
\end{algorithmic}
\end{algorithm}
\BM{well-defined? well-conditioned ?}





\begin{proposition}
Let $\bP^\star = \left(\begin{smallmatrix} \bA & \bC \\ \bC^\top & \bB \end{smallmatrix}\right)$ be the optimal solution of \eqref{eq:ent_bures}. Then $\pi \defeq \Ncal(0, \bP^\star)$ is the optimal solution of \eqref{eq:ent_ot} with $\alpha = \Ncal(0, \bA)$ and $\beta = \Ncal(0, \bB)$.
\end{proposition}\BM{This result is only useful if we wish to introduce entropic Bures without relying on the Sinkhorn iterations with quadratic potentials, as in \cref{subsec:ent_ot_gaussians}}

\begin{proof}
It is sufficient to prove\BM{add ref} that $\pi$ is of the form $\d\pi(x,y) = \exp(\tfrac{1}{\varepsilon}(f(x) + g(y) - \| x - y\|^2)) \d\alpha(x)\d\beta(y)$ and has the right marginals. The latter point is obvious, let us prove the former. Let $\bU$, $\bV$ be defined as in \Cref{eq:change-of-variable}, and $\exp(f / \varepsilon) \propto G_{\bU}$ and $\exp(g / \varepsilon) \propto G_{\bV}$. Then 
%
\begin{align}
    &\exp(\tfrac{1}{\varepsilon}(f(x) + g(y) - \| x - y\|^2)) \d\alpha(x)\d\beta(y) \\
    &\quad= G_{\bU}(x)G_{\bA}(x) e^{-\frac{\| x- y\|^2}{2\sigma^2}}G_{\bV}(y)G_{\bB}(y)\\
    &\quad= G_{\bU \oplus \bA}(x) e^{-\frac{\| x- y\|^2}{2\sigma^2}}G_{\bV \oplus \bB}(y)\\
    &\quad=  e^{-\tfrac{1}{2}(x,y)^\top \bH^{-1}(x,y)},
\end{align}
%
with
%
\begin{align}
    \bH^{-1} &= 
    \begin{pmatrix} 
        \bU^{-1} + \bA^{-1} + \frac{1}{\sigma^2} \Id & - \frac{1}{\sigma^2} \Id \\
         -  \frac{1}{\sigma^2} \Id  & \bV^{-1} + \bB^{-1} + \frac{1}{\sigma^2} \Id\\
    \end{pmatrix},
\end{align}
%
and hence, using \Cref{eq:change-of-variable}
\begin{align}
    \bH^{-1} &= 
    \begin{pmatrix} 
      \bA^{-1} + \frac{1}{\sigma^2} \bG^{-1} & - \frac{1}{\sigma^2} \Id \\
         -  \frac{1}{\sigma^2} \Id  & \bB^{-1} + \frac{1}{\sigma^2} \bF^{-1}\\
    \end{pmatrix},
\end{align}
%
and using \Cref{eq:bures-sinkhorn-iterations},
%
\begin{align}
    \bH &= \begin{pmatrix}
        \bA & \bA \bG^{-1} \\
          \bG^{-1}\bA & \bB\\
    \end{pmatrix},
\end{align}
%
and we conclude from \Cref{eq:primal-dual}.
\end{proof}


%unproven proposition
\begin{proposition}
\label{prop:convergence}
Assume $\alpha, \beta$ are centered sub-Gaussian measures i.e $\exists \zeta_0 > 0$ such that $\Esp_{\alpha}e^{\frac{\|\bX\|^2}{2d\zeta_0}} \leq 2$ and $\Esp_{\beta}e^{\frac{\|\bX\|^2}{2d\zeta_0}} \leq 2$. Given an initial point $(f_0,
g_0)$ such that for all $x$ it holds $|f_0(x)| \leq \|x\|^2$, the iterations \eqref{eq:alg_sinkhorn} are well-defined and converge towards a pair of optimal dual potentials $(f, g)$.  \hicham{Not proven yet -- abandonned for the moment}
\end{proposition}
\begin{proof}
Using the results derived by \citet{mena19} on sub-Gaussian measures, we adapt the proof of \citet{sejourne19} to the non-compact setting. To do so, we use the extended version of Arzela-Ascoli: ``If a sequence of functions $h_n: \RR^d \to \RR$ is equicontinuous and pointwise bounded, then there exists a subsequence $h_{n_j}$ which converges uniformly on compact sets to a continuous function $h$.''
\begin{itemize}
    \item Well-posedness of $(f_n, g_n)_n$. 
    Let $x, y \in \RR^d$. It holds:
      $\frac{-\|x-y\|^2 + f_0(x)}{2\sigma^2} \leq \frac{\|x\|^2}{2\sigma^2}$, therefore using the sub-Gaussianity assumption 
    \item Pointwise boundedness of $(f_n)_n$. Let $x \in \RR^d$. We are going to show that there exists $M > 0$ such that for all $n \geq 0 \quad |f_n(x)| \leq M\|x\|^2$ using a proof by induction.
    \item Equicontinuity of $(f_n)_n$.
\end{itemize}
\end{proof}


==> sections/hellinger.tex <==
\section{Unbalanced OT}
Let $\alpha, \beta \in \Mcal^+_2(\RR^d)$ with finite integration masses $m_\alpha = \alpha(\RR^d)$ and $m_\beta=\beta(\RR^d)$. We define Unbalanced OT (UOT) as:
\begin{equation}
\label{eq:def-uot-0}
    \UOT(\alpha, \beta) \defeq \inf_{\pi \in \Mcal^+_2(\Xcal\times \Ycal)} \int_{\RR^{d}\times \RR^d} \| x - y \|^2 \dd\pi(x,y)
    + \gamma \KL(\pi_1\Vert \alpha) + \gamma \KL(\pi_2\Vert \beta).
\end{equation}
where $\gamma > 0$ is a hyperparameter controlling the distance between the marginals $\pi_1$, $\pi_2$ and the measures $\alpha, \beta$.

On one hand, a necessary condition for the KL terms of the loss function \eqref{eq:def-uot-0} to be finite is $\pi_1 \ll \alpha$ and $\pi_2 \ll \beta$. On the other hand, for any borel sets A, B $\subset \RR^d$ it holds: $(\pi_1\otimes\pi_2)(A\times B) = 0 \Rightarrow \pi_1(A) = 0$ or $ \pi_2(B) = 0 \Rightarrow \pi(A\times\RR^d) = 0$ or $\pi(\RR^d\times B) = 0 \Rightarrow \pi(A\times B) = 0$ (by inclusion). Therefore, $\pi$ must verify: $\pi \ll \pi_1 \otimes \pi_2 \ll \alpha\otimes\beta$. 

\hicham{\subsection{Discrete case}}
\begin{equation}
    \UOT(\alpha, \beta) \defeq \inf_{\pi \in \RR^{n\times n}} \langle C, \pi\rangle 
    + \gamma \KL(\pi \mathds 1 \Vert \alpha) + \gamma \KL(\pi^\top \mathds 1\Vert \beta).
\end{equation}
KKT: $\exists Z \in \RR^{n \times n}$ such that:
\begin{align*}
    \left{\begin{array}{ll}
          C_{ij} + \gamma \log(\frac{(\pi\mathds 1)_i}{a_i}) + \gamma \log(\frac{(\pi^\top\mathds 1)_j}{b_j}) - Z_{ij} = 0 \\
          \pi_{ij} \geq 0 \\
          Z_{ij} \geq 0
\end{align*}


\hicham{\subsection{Gaussian plan}}
Let $\mathfrak{BH}_\gamma(\bA, \bB)$ denote the unbalanced optimal transport \eqref{eq:unbalanced_ot} between centered Gaussian measures, with entropic regularization:\BM{TODO: argument that shows that optimal plan is indeed Gaussian.}

\begin{align}\label{eq:unbalanced_bures}
    \underset{\left(\begin{smallmatrix} \bX_1 & \bX_3 \\ \bX_3^T & \bX_2 \end{smallmatrix}\right) \geq 0}{\min} &\Big\{\tr{\bX_1} + \tr{\bX_2} - 2 \tr{\bX_3}\\
    &+ \sigma^2\Big(\tr(\bA^{-1}\bX_1 + \bB^{-1}\bX_2) - 2d\\ &
    +  \log\det \bA + \log\det \bB - \log\det\left(\begin{smallmatrix} \bX_1 & \bX_3 \\ \bX_3^T & \bX_2 \end{smallmatrix}\right)\Big)\nonumber\\
    & + \gamma\KL(\bX_1\Vert\bA) + \gamma\KL(\bX_2\Vert\bB)\Big\}.
\end{align}
%
We have that \eqref{eq:unbalanced_bures} is equivalent to
%
\begin{align*}
   \underset{\bX_1, \bX_2 \geq 0}{\min} \Big\{& \gamma\KL(\bX_1\Vert\bA) + \gamma\KL(\bX_2\Vert\bB)  \\
   & + \underset{\bX_3 : \left(\begin{smallmatrix} \bX_1 & \bX_3 \\ - 2 \bX_3^T & \bX_2 \end{smallmatrix}\right)\geq 0}{\min} \tr{\bX_1} + \tr{\bX_2} - 2 \tr{\bX_3} \\
   &+ \sigma^2\Big(\tr(\bA^{-1}\bX_1 + \bB^{-1}\bX_2) - 2d \\ &
    +  \log\det \bA + \log\det \bB - \log\det\left(\begin{smallmatrix} \bX_1 & \bX_3 \\ \bX_3^T & \bX_2 \end{smallmatrix}\right)\Big)\Big\}\\
\end{align*}
%
and hence, using 

\begin{align}
    \mathfrak{BH}_{\sigma^2, \gamma}(\bA, \bB) =  \underset{\bX_1, \bX_2 \geq 0}{\min} \Bures_{\sigma^2}(\bX_1, \bX_2) + \gamma\KL(\bX_1\Vert\bA) + \gamma\KL(\bX_2\Vert\bB) 
\end{align}
%
\boris{This is still valid in the $\sigma = 0$ case.}
%
\paragraph{Bures-Hellinger Distance ($\sigma^2 = 0$)}
%
% \begin{align}\label{eq:bures_hell_def}
%     \underset{\left(\begin{smallmatrix} \bX_1 & \bX_3 \\ \bX_3^T & \bX_2 \end{smallmatrix}\right) \geq 0}{\min} &\Big\{\tr{\bX_1} + \tr{\bX_2} - 2 \tr{\bX_3}\nonumber\\
%     &+ \gamma\KL(\bX_1\Vert\bA) + \gamma\KL(\bX_2\Vert\bB)\Big\}.
% \end{align}
% %
% We have that \eqref{eq:bures_hell_def} is equivalent to
% %
% \begin{align*}
%   \underset{\bX_1, \bX_2 \geq 0}{\min} \Big\{&\tr{\bX_1} + \tr{\bX_2} - 2 \underset{\bX_3 : \left(\begin{smallmatrix} \bX_1 & \bX_3 \\ \bX_3^T & \bX_2 \end{smallmatrix}\right)\geq 0}{\max} \tr{\bX_3}\\
%   &+ \gamma\KL(\bX_1\Vert\bA) + \gamma\KL(\bX_2\Vert\bB) \Big\}.
% \end{align*}
% %
% Finally, using that
% \begin{align*}
% \underset{\bX_3 : \left(\begin{smallmatrix} \bX_1 & \bX_3 \\ \bX_3^T & \bX_2 \end{smallmatrix}\right)\geq 0}{\max} \tr{\bX_3} = \tr(\bX_1\rt\bX_2\bX_1\rt)\rt,    
% \end{align*} 
% %
% (see \citep{bhatia2019}) we get 
%
\begin{align}
    \mathfrak{BH}_\gamma(\bA, \bB) =  \underset{\bX_1, \bX_2 \geq 0}{\min} \Bures(\bX_1, \bX_2) + \gamma\KL(\bX_1\Vert\bA) + \gamma\KL(\bX_2\Vert\bB) 
\end{align}
%
\boris{Using \Cref{eq:primal_K}, we should get the same type of formulation with regularization.}


In particular, at the optimum we have
%
\begin{align*}
    &2(\Id - \bT^{\bX_1\bX_2}) - \tfrac{\gamma}{2}\bX_1^{-1} + \tfrac{\gamma}{2}\bA^{-1} = 0\\
    &2(\Id - \bT^{\bX_2\bX_1}) - \tfrac{\gamma}{2}\bX_2^{-1} + \tfrac{\gamma}{2}\bB^{-1} = 0
\end{align*}

\boris{TODO: look at the dual}



